Occlusions, Motion and Depth Boundaries with a Generic Network for Disparity, Optical Flow or Scene Flow Estimation

Occlusions play an important role in disparity and optical flow estimation, since matching costs are not available in occluded areas and occlusions indicate depth or motion boundaries. Moreover, occlusions are relevant for motion segmentation and scene flow estimation. In this paper, we present an efficient learning-based approach to estimate occlusion areas jointly with disparities or optical flow. The estimated occlusions and motion boundaries clearly improve over the state-of-the-art. Moreover, we present networks with state-of-the-art performance on the popular KITTI benchmark and good generic performance. Making use of the estimated occlusions, we also show improved results on motion segmentation and scene flow estimation.

==> motionboundaries.tex <==
\newcommand{\galleryRowSintel}[4]{\vspace*{-0.075cm} \includegraphics[width=0.2\textwidth]{images/#1} & \includegraphics[width=0.2\textwidth]{images/#2} & \includegraphics[width=0.2\textwidth]{images/#3} & \includegraphics[width=0.2\textwidth]{images/#4} \tabularnewline
}
  \resizebox{\linewidth}{!}{%
    \setlength{\tabcolsep}{0.7pt}%
    \begin{tabular}{cccc}%
\galleryRowSintel{motionboundaries/img0.png}{motionboundaries/img1.png}{motionboundaries/gt_mb_thick.png}{motionboundaries/pred_mb_thick.png}%
\galleryRowSintel{motionboundaries/img02.png}{motionboundaries/img12.png}{motionboundaries/gt_mb2_thick.png}{motionboundaries/pred_mb2_thick.png}%
\galleryRowSintel{motionboundaries/img03.png}{motionboundaries/img13.png}{motionboundaries/gt_mb3_thick.png}{motionboundaries/pred_mb3_thick.png}%
    \end{tabular}%
  }% 

==> occlusion.tex <==
\newcommand{\galleryRowSintel}[6]{\vspace*{-0.075cm} \includegraphics[width=0.2\textwidth]{images/#1} & \includegraphics[width=0.2\textwidth]{images/#2} & \includegraphics[width=0.2\textwidth]{images/#3} & \includegraphics[width=0.2\textwidth]{images/#4} & \includegraphics[width=0.2\textwidth]{images/#5} & \includegraphics[width=0.2\textwidth]{images/#6} \tabularnewline
}
  \resizebox{\linewidth}{!}{%
    \setlength{\tabcolsep}{0.7pt}%
    \begin{tabular}{cccccc}%
\galleryRowSintel{occlusion/img0.png}{occlusion/img1.png}{occlusion/gt_occ.png}{occlusion/pred_occ.png}{occlusion/mrflow_occ.png}{occlusion/s2d_occ.png}%
\galleryRowSintel{occlusion/img02.png}{occlusion/img12.png}{occlusion/gt_occ2.png}{occlusion/pred_occ2.png}{occlusion/mrflow_occ2.png}{occlusion/s2d_occ2.png}%
\galleryRowSintel{occlusion/img03.png}{occlusion/img13.png}{occlusion/gt_occ3.png}{occlusion/pred_occ3.png}{occlusion/mrflow_occ3.png}{occlusion/s2d_occ3.png}%
    \end{tabular}%
  }% 

==> tables/compare_table/compare_tab_flow_bkp.tex <==
\newcommand{\rowline} {\hhline{|~||~~~~|~~~~||~|}} 
\newcommand{\headerline} {\hhline{|=||====|====||=|}} 

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l||cccc|cccc||c|}
% --- begin header
\hhline{|-||----|----||-|}
\textbf{Method} 
&\multicolumn{2}{c}{\textbf{Sintel}} 
&\multicolumn{2}{c|}{\textbf{Sintel}}
&\multicolumn{2}{c}{\textbf{KITTI}}
&\multicolumn{2}{c||}{\textbf{KITTI}}
%&\multicolumn{2}{c||}{\textbf{Middlebury}}
& \textbf{Runtime} \\

%empty
&\multicolumn{2}{c}{(clean)} 
&\multicolumn{2}{c|}{(final)}
&\multicolumn{2}{c}{(2012)}
&\multicolumn{2}{c||}{(2015)}
%&&
& (s)
\\
\hhline{|~||~~~~|~~~~|~~||~|}
%empty
&\multicolumn{2}{c}{AEE} 
&\multicolumn{2}{c|}{AEE} 
& \textit{AEE} & \textit{OUT-noc}  
& \textit{AEE} & \textit{F1-all} 
%&\multicolumn{2}{c||}{AEE} 
&  %empty
\\
\hhline{|~||~~~~|~~~~|~~||~|}
%empty
& \textit{train} & \textcolor{black}{\textit{test} }
& \textit{train} & \textcolor{black}{\textit{test} }
& \textit{train} & \textcolor{black}{\textit{test} }
& \textit{train} & \textcolor{black}{\textit{test} }
%& \textit{train} & \textcolor{red}{\textit{test} }
& % empty   
\\
\headerline 
% --- end header

% ########## Standard approaches ##############
\textbf{Standard}
&&&&&&&&&\\
\headerline 


% --- begin method
EpicFlow~\cite{epicflow}
& ${2.27}$  & $4.12$  % Sintel (clean) train,test
& ${3.56}$  & $6.29$  % Sintel (final) train,test
& $\mathbf{3.09}$  & $7.88\%$ % KITTI 12 train,test
& ${9.27}$  & $26.29\%$	  % KITTI 15 train,test
%& $0.31$  & $0.39$  % Middlebury train,test
& $42$   % runtime 
\\
\rowline 
% --- end method

% --- begin method
FlowfieldsCNN~\cite{flowfieldscnn}
& -  & $3.78$ % Sintel (clean) train,test
& -  & $5.36$  % Sintel (final) train,test
& -  & ${4.89\%}$ % KITTI 12 train,test
& -  & $18.68\%$	  % KITTI 17 train,test
%& -  & -  % Middlebury train,test
& $23$  % runtime
\\
\rowline 
% --- end method

%--- begin method
DCFlow~\cite{dcflow}
& -  & $\mathbf{3.54}$  % Sintel (clean) train,test
& -  & ${5.12}$ % Sintel (final) train,test
& -  & -  % KITTI 12 train,test
& -  & ${14.86\%}$	  % KITTI 15 train,test
%& -  & -  % Middlebury train,test
& $\pz{9}$
\\

\rowline 
% --- end method

% ########## END Standard approaches ##############

% ########## CNN approaches ##############
\headerline 
\textbf{CNN based}
&&&&&&&&& \\
\headerline 
%% --- begin methodFlowNet2
FlowNet2~\cite{flownet2}
& $\mathbf{2.02}$  & ${3.96}$  % Sintel (clean) train,test
& $\mathbf{3.14}$  & $6.02$  % Sintel (final) train,test
& ${4.09}$  & -       % KITTI 12 train,test
& ${10.06}$ & -       % KITTI 15 train,test
%& $0.35$  & $0.52$  % Middlebury train,test
& $0.123$  
\\
% --- end method 
%% --- begin method
FlowNet2-ft~\cite{flownet2}
& $(1.45)$  & $4.16$  % Sintel (clean) train,test
& $(2.01)$  & $5.74$  % Sintel (final) train,test
& $(1.28)$  & -  % KITTI 12 train,test
& $(2.30)$  & $11.48\%$  % KITTI 15 train,test
%& $0.35$  & -  % Middlebury train,test
& $0.123$  
\\
% --- end method 
%% --- begin method
SpyNet~\cite{spynet}
& $4.12$  & $6.69$ % Sintel (clean) train,test
& $5.57$  & $8.43$ % Sintel (final) train,test
& $9.12$  & -  % KITTI 12 train,test
& -       & -  % KITTI 15 train,test
%& -  & -  % Middlebury train,test
& $\mathbf{0.016}$  
\\
% --- end method 
%% --- begin method
SpyNet-ft~\cite{spynet}
& $(3.17)$ & $6.64$ % Sintel (clean) train,test
& $(4.32)$ & $8.36$  % Sintel (final) train,test
& $(4.13)$ & $12.31\%$  % KITTI 12 train,test
& -        &  $35.07\%$  % KITTI 15 train,test
%& - & -  % Middlebury train,test
& $\mathbf{0.016}$  
\\
% --- end method 
%--- begin method
PWC-Net~\cite{pwcnet}
& $2.55$  & -  % Sintel (clean) train,test
& $3.93$  & -  % Sintel (final) train,test
& $4.14$  & -  % KITTI 12 train,test
& $10.35$ & $33.67\%$ % KITTI 15 train,test
%& -  & -  % Middlebury train,test
& $0.030$  
\\
%% --- begin method
PWC-Net-ft~\cite{pwcnet}
& $(2.02)$  & $4.39$   % Sintel (clean) train,test
& $(2.08)$  & $\mathbf{5.04}$  % Sintel (final) train,test
& -         & ${4.22\%}$  % KITTI 12 train,test
& $(2.16)$  & $9.80\%$	  % KITTI 15 train,test
%& -       & -  % Middlebury train,test
& $0.030$  
\\
% --- end method 

% ########## END CNN  approaches ##############

\headerline 
% ########## Joint Estimation ##############
\textbf{With joint occ est.}
&&&&&&&&&\\
%\hhline{|=||====|====|==||==|}
\headerline 
% --- begin method
MirrorFlow~\cite{mirrorflow}
& -  & $3.32$  % Sintel (clean) train,test
& -  & $6.07$  % Sintel (final) train,test
& -  & $4.38\%$  % KITTI 12 train,test
& -  & $10.29\%$  % KITTI 15 train,test
%& -  & -  % Middlebury train,test
& $\pz\pz660$
\\
% --- end method
% --- begin method
S2D flow~\cite{affine_s2d}
& -  & $18.48$  % Sintel (clean) train,test
& -  & $6.82$  % Sintel (final) train,test
& -  & -  % KITTI 12 train,test
& -  & -  % KITTI 15 train,test
%& -  & $0.35$  % Middlebury train,test
& $\pz2280$ % 38 mins! 
\\
% --- end method

% --- begin method
Our FlowNet-CSS
%& ${2.06}$  & $3.94$  % Sintel (clean) train,test caffe
& $\tct{2.08}$  & $3.94$  % Sintel (clean) train,test tf
%& $3.57$  &  $6.03$  % Sintel (final) train,test caffe
& $\tct{3.61}$  &  $6.03$  % Sintel (final) train,test tf
%& $3.52$  & -  % KITTI 12 train,test caffe
& $\tct{3.69}$  & -  % KITTI 12 train,test tf
%& $\mathbf{9.13}$  & -  % KITTI 15 train,test caffe
& $\tct{\mathbf{9.33}}$  & -  % KITTI 15 train,test tf
& $0.077$     
\\
% --- end method
% --- begin method
Our FlowNet-CSS-ft
%& $(1.46)$  & $4.35$ % Sintel (clean) train,test caffe
& $(\tct{1.47})$  & $4.35$ % Sintel (clean) train,test tf
%& $(2.12)$  & $5.67$% Sintel (final) train,test caffe
& $(\tct{2.12})$  & $5.67$% Sintel (final) train,test tf
%& $(0.99)$  & $\mathbf{3.45}\%$  % KITTI 12 train,test caffe
& $(\tct{1.19})$  & $\mathbf{3.45}\%$  % KITTI 12 train,test
%& $(1.45)$  & $\mathbf{8.60}\%$  % KITTI 15 train,test
& $(\tct{1.79})$  & $\mathbf{8.60}\%$  % KITTI 15 train,test
%& ?  & -  % Middlebury train,test
& $0.077$     
%& $0.094$     
\\
% --- end method
% --- begin method
Our FlowNet-css 
%& $2.63$  & -  % Sintel (clean) train,test caffe
& $\tct{2.65}$  & -  % Sintel (clean) train,test
%& $4.04$  & -  % Sintel (final) train,test caffe
& $\tct{4.05}$  & -  % Sintel (final) train,test 
%& $4.91$  & -  % KITTI 12 train,test caffe
& $\tct{5.05}$  & -  % KITTI 12 train,test
%& $11.45$ &    % KITTI 15 train,test caffe
& $\tct{11.74}$ &    % KITTI 15 train,test
%&  ?      & -  % Middlebury train,test
& $0.020$  
\\
% --- end method

% ########## END Standard approaches ##############
\hhline{|-||----|----||-|}
\end{tabular}%
}


==> tables/results_table.tex <==
\onecolumn
\resizebox{\textwidth}{!}{%
      %% This table needs the {hhline} package
      \begin{tabular}{|c|l||cc|cc||cc|ccc||cc||cc|}%
        \hhline{|-|-||--|--T--|---T--||--|}%
               & Method
               & \multicolumn{2}{c|}{Sintel \textit{clean}}%
               & \multicolumn{2}{c||}{Sintel \textit{final}}%
               & \multicolumn{2}{c|}{KITTI 2012}%
               & \multicolumn{3}{c||}{KITTI 2015}%
               & \multicolumn{2}{c||}{Middlebury}%
               & \multicolumn{2}{c|}{Runtime}%
               \\%
               
               &
               & \multicolumn{2}{c|}{AEE}%
               & \multicolumn{2}{c||}{AEE}%
               & \multicolumn{2}{c|}{AEE}%
               & AEE
               & Fl-all
               & Fl-all
               & \multicolumn{2}{c||}{AEE}%
               & \multicolumn{2}{c|}{ms per frame}%
               \\%
               
               &
               & \textit{train} & \textit{test}%
               & \textit{train} & \textit{test}%
               & \textit{train} & \textit{test}%
               & \textit{train}&\textit{train}&\textit{test}%
               & \textit{train} & \textit{test}%
               & CPU & GPU%
               \\%
               
        \hhline{|=|=||==|==#==|===#==||==|}%
        % flow header
        \multicolumn{15}{|l|}{Optical flow}\\
        \hhline{|=|=||==|==#==|===#==||==|}%
        % end flow heder 
        \multirow{4}{*}{\rotatebox[origin=c]{90}{Others}} 
        &
        FlowNet2-CSS 
        & $2.10$ & -- %Sintel-clean
        & $3.23$ & -- %Sintel-final
        & $\pz\textbf{3.55}$ & -- %Kitti-2012
        & $\textbf{\pz8.94}$ & $29.77\%$ & -- %Kitti-2015
        & $0.44$ & -- %Middlebury-AEE
        %& $\pz7.25$ & -- %Middlebury-AAE
        & -- & $\pz\pz\pz69$%Sintel-runtime
        \\%
        &
        FlowNet2     
        & $\textbf{2.02}$ & $\textbf{3.96}$ %Sintel-clean
        & $\textbf{3.14}$ & $6.02$ %Sintel-final
        & $\pz4.09$  & --  %Kitti-2012
        & $10.06$ & $30.37\%$ & -- %Kitti-2015
        & $\textbf{0.35}$ & $\textbf{0.52}$ %Middlebury-AEE
        %& \cellcolor{gray!15}$\pz\textbf{4.59}$ & \cellcolor{gray!15}$\textbf{5.87}$ %Middlebury-AAE
        & -- & $\pz\pz123$%Sintel-runtime
        \\%
        % kitti timing: 0.128

        % net: 60a0cS_sintel_submit2 (nikolaus: pls confirm)
        &
        FlowNet2-ft-sintel  
        & ($1.45$) & $4.16$ %Sintel-clean
        %\textcolor{cyan}{$2.73$} / \textcolor{cyan}{$2.84$} & \tce{\todo} 
        & ($2.01$) & $\textbf{5.74}$ %Sintel-final 
        %\textcolor{cyan}{$4.23$} / \textcolor{cyan}{$4.09$} & \tce{\todo} 
        & $\pz3.61$ & -- %Kitti-2012
        & $\pz9.84$ & $\textbf{28.20\%}$ & -- %Kitti-2015
        & $0.35$ & -- %Middlebury-AEE
        %& $\pz4.55$ & -- %Middlebury-AAE
        & -- & $\pz\pz123$%Sintel-runtime
        \\%

        &
        FlowNet2-ft-kitti
        & $3.43$ & -- %Sintel-clean
        & $4.66$ & -- %Sintel-final
        & $\pz$($1.28$) & \textbf{1.8} %Kitti-2012
        & $\pz$($2.30$) & $\pz$($8.61\%$) & $\textbf{11.48\%}$ %Kitti-2015
        & $0.56$ & -- %Middlebury-AEE
        %& $\pz7.07$ & -- %Middlebury-AAE
        & -- & $\pz\pz123$%Sintel-runtime
        \\%
        % kitti timing: 0.128
        \hhline{|-|-||--|--|--|---|--||--|}%
        \multirow{3}{*}{\rotatebox[origin=c]{90}{FN-Bi}} 
        &
        FlowNetBi 
        & $2.27$  & -- %Sintel-clean
        & $3.83$ & -- %Sintel-final
        & $\pz 4.51$     & -- %Kitti-2012
        & $\pz10.60$     & -- & -- %Kitti-2015
        & $?$     & -- %Middlebury-AEE
        %& $\pz7.25$ & -- %Middlebury-AAE
        & -- & $\pz\pz135$%Sintel-runtime
        \\%
        &
        FlowNetBiSlim
        &  $2.76$ & -- %Sintel-clean
        %\textcolor{cyan}{$2.73$} / \textcolor{cyan}{$2.84$} & \tce{\todo} 
        &  $4.12$ & -- %Sintel-final 
        %\textcolor{cyan}{$4.23$} / \textcolor{cyan}{$4.09$} & \tce{\todo} 
        &  $5.74$ & -- %Kitti-2012
        &  $12.26$ & $$ & -- %Kitti-2015
        &  $$ & -- %Middlebury-AEE
        %& $\pz4.55$ & -- %Middlebury-AAE
        & -- & $\pz\pz108$%Sintel-runtime
        \\%

        &
        FlowNetBiSlimFast
        & $$ & -- %Sintel-clean
        & $$ & -- %Sintel-final
        & $$ & $2.4$ %Kitti-2012
        & $?$  & $?$ & $25.24\%$ %Kitti-2015
        & $?$ & -- %Middlebury-AEE
        %& $\pz7.07$ & -- %Middlebury-AAE
        & -- & $?$%Sintel-runtime
        \\%
        % kitti timing: 0.128
        \hhline{|-|-||--|--|--|---|--||--|}%
        \multicolumn{15}{|l|}{Disparity}\\
        \hhline{|-|-||--|--|--|---|--||--|}%        
       
        %\multirow{4}{*}{\rotatebox[origin=c]{90}{Others}} 
        &
        DispNetC  \cite{dispnet}
        & $5.66$ & -- %Sintel-clean
        & $-$ & -- %Sintel-final
        & $1.75$ & -- %Kitti-2012
        & $1.59$ & -- & -- %Kitti-2015
        & -- & -- %Middlebury-AEE
        %& $\pz7.25$ & -- %Middlebury-AAE
        & -- & $?$%Sintel-runtime
        \\%
        % &
        % CRL  
        % & $-$ & -- %Sintel-clean
        % & $-$ & -- %Sintel-final
        % & $?$ & -- %Kitti-2012
        % & $?$ & $?$ & -- %Kitti-2015
        % & $?$ & -- %Middlebury-AEE
        % %& $\pz7.25$ & -- %Middlebury-AAE
        % & -- & $?$%Sintel-runtime
        % \\%
        % &
        % GC-Net
        % & ($?$) & $?$ %Sintel-clean
        % %\textcolor{cyan}{$2.73$} / \textcolor{cyan}{$2.84$} & \tce{\todo} 
        % & ($?$) & $?$ %Sintel-final 
        % %\textcolor{cyan}{$4.23$} / \textcolor{cyan}{$4.09$} & \tce{\todo} 
        % & $?$ & -- %Kitti-2012
        % & $?$ & $?$ & -- %Kitti-2015
        % & $?$ & -- %Middlebury-AEE
        % %& $\pz4.55$ & -- %Middlebury-AAE
        % & -- & $?$%Sintel-runtime
        % \\%
        % &
        % L-ResMatch
        % & ($?$) & $?$ %Sintel-clean
        % %\textcolor{cyan}{$2.73$} / \textcolor{cyan}{$2.84$} & \tce{\todo} 
        % & ($?$) & $?$ %Sintel-final 
        % %\textcolor{cyan}{$4.23$} / \textcolor{cyan}{$4.09$} & \tce{\todo} 
        % & $?$ & -- %Kitti-2012
        % & $?$ & $?$ & -- %Kitti-2015
        % & $0.35$ & -- %Middlebury-AEE
        % %& $\pz4.55$ & -- %Middlebury-AAE
        % & -- & $?$%Sintel-runtime
        % \\ 
        
        \hhline{|-|-||--|--|--|---|--||--|}%
        
         \multirow{4}{*}{\rotatebox[origin=c]{90}{DN-Bi}} 
        &
        DispNetBi 
        & $3.23$ & -- %Sintel-clean
        & $4.75$ & -- %Sintel-final
        & $1.31$ & -- %Kitti-2012
        & $1.37$ & $1.67$ & -- %Kitti-2015
        & $?$ & -- %Middlebury-AEE
        & -- & $\pz\pz\pz88$%Sintel-runtime
        \\%
        &
        DispNetBiSlim
        & $3.28$ & -- %Sintel-clean
        & $5.04$ & -- %Sintel-final 
        & $1.49$ & -- %Kitti-2012
        & $1.62$ & $2.41$ & %Kitti-2015
        & $?$    & -- %Middlebury-AEE
        & -- & $\pz\pz\pz77$%Sintel-runtime
        \\ 
        &
        DispNetBiKitti
        & $5.14$ & -- %Sintel-clean
        & $7.27$ & -- %Sintel-final 
        %& $0.81$ & -- %Kitti-2012
        & -- & -- %Kitti-2012
        %& $0.89$ & $0.59$ & -- %Kitti-2015
        & -- & -- & -- %Kitti-2015
        & $$ & -- %Middlebury-AEE
        & -- & $\pz\pz\pz 88$%Sintel-runtime
        \\%
        &
        DispNetBiSlimFast
        & $3.51$ & -- %Sintel-clean
        & $5.20$ & -- %Sintel-final
        & $1.48$ & ? %Kitti-2012
        & $1.55$  & $2.18$ & $TBA$ %Kitti-2015
        & $TBA$ & -- %Middlebury-AEE
        & -- & $\pz\pz\pz 58$%Sintel-runtime
        \\%
        % kitti timing: 0.128
        \hhline{|-|-||--|--|--|---|--||--|}%
      \end{tabular}%
    }%
\twocolumn

==> teaser.tex <==
\newcommand{\galleryRowSintel}[2]{\vspace*{-0.075cm} \includegraphics[width=0.2\textwidth]{images/#1} & \includegraphics[width=0.2\textwidth]{images/#2} \tabularnewline
}
  \resizebox{\linewidth}{!}{%
    \setlength{\tabcolsep}{0.7pt}%
    \begin{tabular}{cc}%
\galleryRowSintel{teaser/img0.png}{teaser/img1.png}%
\galleryRowSintel{teaser/pred.png}{teaser/occ.png}%
\galleryRowSintel{teaser/conf.png}{teaser/mb.png}%
    \end{tabular}%
  }% 
